PUPS: Point Cloud Unified Panoptic Segmentation

Point cloud panoptic segmentation is a challenging task that seeks a holistic solution for both semantic and instance segmentation to predict groupings of coherent points. Previous approaches treat semantic and instance segmentation as surrogate tasks, and they either use clustering methods or bounding boxes to gather instance groupings with costly computation and hand-crafted designs in the instance segmentation task. In this paper, we propose a simple but effective point cloud unified panoptic segmentation (PUPS) framework, which use a set of point-level classifiers to directly predict semantic and instance groupings in an end-to-end manner. To realize PUPS, we introduce bipartite matching to our training pipeline so that our classifiers are able to exclusively predict groupings of instances, getting rid of hand-crafted designs, e.g. anchors and Non-Maximum Suppression (NMS). In order to achieve better grouping results, we utilize a transformer decoder to iteratively refine the point classifiers and develop a context-aware CutMix augmentation to overcome the class imbalance problem. As a result, PUPS achieves 1st place on the leader board of SemanticKITTI panoptic segmentation task and state-of-the-art results on nuScenes.

==> tables/ablation_feature_dim.tex <==
\begin{table}[htbp]\small
\begin{center}
\caption{Ablation study of encoder feature dimension on validation set of SemanticKITTI. All scores are in [\%].}
\setlength{\tabcolsep}{2mm}
\centering
\label{tab:ablation_feature_dim}
\begin{tabular}{c|ccc}
\toprule
Feature Dimension & PQ              & SQ              & RQ             \\
\midrule
32                & $62.4$          & $76.1$          & $72.2$           \\
64                & $62.7$          & $80.5$          & $73.0$           \\
128               & $\mathbf{64.4}$ & $\mathbf{81.5}$ & $\mathbf{74.1}$\\
256               & $62.0$          & $80.2$          & $71.9$           \\

\bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/ablation_voxel_size.tex <==
\begin{table}[htbp]\small
\begin{center}
\caption{Ablation study of voxel size on validation set of SemanticKITTI. All scores are in [\%].}
\setlength{\tabcolsep}{2mm}
\centering
\label{tab:ablation_voxel_size}
\begin{tabular}{c|ccc}
\toprule
Voxel Size (cm)    & PQ              & SQ              & RQ             \\
\midrule
2.5                & $62.6$            & $79.3$            & $72.6$           \\
5                  & $\mathbf{64.4}$   & $\mathbf{81.5}$   & $\mathbf{74.1}$\\
7.5                & $56.3$            & $77.5$            & $67.0$           \\
10                 & $56.3$            & $77.5$            & $67.0$           \\

\bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/contextual_points.tex <==
\begin{table}[htbp]\small
\begin{center}
\caption{Contextual classes for \emph{thing} classes and some \emph{stuff} classes of SemanticKITTI}
\setlength{\tabcolsep}{2.4mm}
\centering
\label{tab:contextual_points}
\begin{tabular}{l|l}
\toprule
Instance Class    & Contextual Class \\
\midrule
car               & road, parking \\
bicycle           & sidewalk, other-ground \\
motorcycle        & sidewalk, other-ground \\
truck             & road, parking \\
other-vehicle     & road, parking, other-ground \\
person            & road, parking, sidewalk, other-ground \\
bicyclist         & road, parking, other-ground \\
motorcyclist      & road, parking, other-ground \\
pole              & sidewalk, other-ground \\
traffic-sign      & pole \\

\bottomrule
\end{tabular}
%\qquad
\begin{center}
% \vspace{-1.5em}
\label{tabepe}
\end{center}
\end{center}
\end{table}

==> tables/nus_test_mean.tex <==
\begin{table*}[htbp]
\begin{center}
\caption{Comparison of LiDAR panoptic segmentation performance on nuScenes test set. C.P., SPV, CYL and $\textrm{(AF)}^2$ refer to CenterPoint~\cite{center-point}, SPVNAS~\cite{spvnas}, Cylinder3D++~\cite{cylinder3d} and $\textrm{(AF)}^2$-S3Net~\cite{AF2S3Net}. All scores are in [\%].}
\label{tab:nus_test_mean}
\footnotesize
\begin{tabular}
{l|cccc|ccc|ccc|c}
%{p{4.5cm}|p{0.5cm}p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}p{0.5cm}|p{0.6cm}}
\toprule
Method & PQ & PQ$^\dagger$  & SQ & RQ & PQ\textsuperscript{Th} & SQ\textsuperscript{Th} & RQ\textsuperscript{Th} & PQ\textsuperscript{St} & SQ\textsuperscript{St} & RQ\textsuperscript{St} & mIoU  \\
\midrule
%\noalign{\smallskip}\hline\hline\noalign{\smallskip}
% R.Net+ P.P.               & $37.1$ & $45.9$ & $75.9$ & $47.0$ & $20.2$ & $75.2$ & $25.2$ & $49.3$ & $76.5$ & $62.8$ & $52.4$ \\
% LPSAD                     & $38.0$ & $47.0$ & $76.5$ & $48.2$ & $25.6$ & $76.8$ & $31.8$ & $47.1$ & $76.2$ & $60.1$ & $50.9$ \\
PanopticTrackNet          & $51.4$ & $56.2$ & $80.2$ & $63.3$ & $45.8$ & $81.4$ & $55.9$ & $60.4$ & $78.3$ & $75.5$ & $58.0$ \\
% KPC + P.P.                & $44.5$ & $52.5$ & $80.0$ & $54.4$ & $32.7$ & $81.5$ & $38.7$ & $53.1$ & $79.0$ & $65.9$ & $58.8$ \\
% Panoster                  & $52.7$ & $59.9$ & $80.7$ & $64.1$ & $49.4$ & $83.3$ & $58.5$ & $55.1$ & $78.8$ & $68.2$ & $59.9$ \\
EfficientLPS              & $62.4$ & $66.0$ & $83.7$ & $74.1$ & $57.2$ & $83.6$ & $68.2$ & $71.1$ & $83.8$ & $84.0$ & $66.7$ \\
Panoptic-PolarNet         & $63.6$ & $67.1$ & $84.3$ & $75.1$ & $59.0$ & $84.3$ & $69.8$ & $71.3$ & $84.2$ & $83.9$ & $67.0$ \\
SPV + C.P.                & $72.2$ & $76.0$ & $88.5$ & $81.2$ & $71.7$ & $89.7$ & $79.4$ & $73.2$ & $86.4$ & $84.2$ & $76.9$ \\
CYL + C.P.                & $76.5$ & $79.4$ & $89.6$ & $85.0$ & $76.8$ & $91.1$ & $84.0$ & $76.0$ & $87.2$ & $86.6$ & $77.3$ \\
$\textrm{(AF)}^2$ + C.P.  & $76.8$ & $80.6$ & $89.5$ & $85.4$ & $79.8$ & $91.8$ & $86.8$ & $71.8$ & $85.7$ & $83.0$ & $78.8$ \\
Panoptic-PHNet            & $80.1$ & $82.8$ & $91.1$ & $87.6$ & $82.1$ & $93.0$ & $88.1$ & $76.6$ & $87.9$ & $86.6$ & $80.2$ \\
\midrule
\ours (ours) & $\mathbf{62.2}$ & $\mathbf{65.8}$ & $\mathbf{84.2}$ & $\mathbf{72.8}$ & $\mathbf{65.7}$ & $\mathbf{90.6}$ & $\mathbf{72.7}$ & $\mathbf{59.6}$ & $\mathbf{79.5}$ & $\mathbf{73.1}$ & $\mathbf{64.2}$\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> tables/sem_test_classwise.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{2.5pt}
\begin{center}
\caption{Class-wise PQ, SQ, RQ on SemanticKITTI test set. All scores are in [\%].}
        \label{tab:sem_test_classwise}
        \footnotesize
        \begin{tabular}{c|cccccccc|ccccccccccc|c}
            \toprule
            \begin{sideways}Metric\end{sideways} & \begin{sideways}car\end{sideways} & \begin{sideways}truck\end{sideways} & \begin{sideways}bicycle\end{sideways} & \begin{sideways}motorcycle\end{sideways} & \begin{sideways}other vehicle\end{sideways} & \begin{sideways}person\end{sideways} & \begin{sideways}bicyclist\end{sideways} & \begin{sideways}motorcyclist\end{sideways} & \begin{sideways}road\end{sideways} & \begin{sideways}sidewalk\end{sideways} & \begin{sideways}parking\end{sideways} & \begin{sideways}other ground\end{sideways} & \begin{sideways}building\end{sideways} & \begin{sideways}vegetation\end{sideways} & \begin{sideways}trunk\end{sideways} & \begin{sideways}terrain\end{sideways} & \begin{sideways}fence\end{sideways} & \begin{sideways}pole\end{sideways} & \begin{sideways}traffic sign\end{sideways} & \begin{sideways}Mean\end{sideways} \\
            \midrule
            \rowcolor[HTML]{D2FFFF}
            PQ & $90.4$ & $45.9$ & $47.3$ & $70.3$ & $45.1$ & $76.3$ & $80.6$ & $69.8$ & $89.0$ & $68.7$ & $48.7$ & $5.97$ & $85.8$ & $79.5$ & $60.9$ & $46.1$ & $53.4$ & $53.1$ & $64.9$ & $62.2$\\
            SQ & $93.7$ & $93.4$ & $76.0$ & $91.3$ & $92.6$ & $89.4$ & $92.8$ & $95.9$ & $91.9$ & $81.3$ & $76.2$ & $65.0$ & $92.7$ & $84.3$ & $76.7$ & $75.2$ & $76.8$ & $74.2$ & $80.4$ & $84.2$\\
            RQ & $96.5$ & $49.1$ & $62.3$ & $77.1$ & $48.8$ & $85.3$ & $86.8$ & $72.8$ & $96.8$ & $84.4$ & $63.8$ & $9.18$ & $92.6$ & $94.3$ & $79.4$ & $61.2$ & $69.5$ & $71.6$ & $80.7$ & $72.8$ \\
            \bottomrule
        \end{tabular}
    \end{center}
\end{table*}

==> tables/sem_test_classwise_pq.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{1.5pt}
\begin{center}
\caption{Class-wise PQ on SemanticKITTI test set. All scores are in [\%].}
         \label{tab:sem_test_classwise}
         \footnotesize
        \begin{tabular}{l|ccccccccccccccccccc|c}
            \toprule
            Method & \begin{sideways}car\end{sideways} & \begin{sideways}truck\end{sideways} & \begin{sideways}bicycle\end{sideways} & \begin{sideways}motorcycle\end{sideways} & \begin{sideways}other vehicle\end{sideways} & \begin{sideways}person\end{sideways} & \begin{sideways}bicyclist\end{sideways} & \begin{sideways}motorcyclist\end{sideways} & \begin{sideways}road\end{sideways} & \begin{sideways}sidewalk\end{sideways} & \begin{sideways}parking\end{sideways} & \begin{sideways}other ground\end{sideways} & \begin{sideways}building\end{sideways} & \begin{sideways}vegetation\end{sideways} & \begin{sideways}trunk\end{sideways} & \begin{sideways}terrain\end{sideways} & \begin{sideways}fence\end{sideways} & \begin{sideways}pole\end{sideways} & \begin{sideways}traffic sign\end{sideways} & PQ \\
            \midrule
            R.Net + P.P. & $66.9$ & $6.7$ & $3.1$ & $16.2$ & $8.8$ & $14.6$ & $31.8$ & $13.5$ & $90.6$ & $63.2$ & $41.3$ & $6.7$ & $79.2$ & $71.2$ & $34.6$ & $37.4$ & $38.2$ & $32.8$ & $47.4$ & $37.1$\\
            KPC + P.P. & $72.5$ & $17.2$ & $9.2$ & $30.8$ & $19.6$ & $29.9$ & $59.4$ & $22.8$ & $84.6$ & $60.1$ & $34.1$ & $8.8$ & $80.7$ & $77.6$ & $53.9$ & $42.2$ & $49.0$ & $46.2$ & $46.8$ & $44.5$\\
            % LPSAD & $76.5$ & $7.1$ & $6.1$ & $23.9$ & $14.8$ & $29.4$ & $29.7$ & $17.2$ & $90.4$ & $60.1$ & $34.6$ & $5.8$ & $76.0$ & $69.5$ & $30.3$ & $36.8$ & $37.3$ & $31.3$ & $45.8$ & $38.0$ \\
            % PanopticTrackNet & $70.8$ & $14.4$ & $17.8$ & $20.9$ & $27.4$ & $34.2$ & $35.4$ & $7.9$ & $91.2$ & $66.1$ & $50.3$ & $10.5$ & $81.8$ & $75.9$ & $42.0$ & $44.3$ &  $42.9$ & $33.4$ & $51.1$ & $43.1$ \\
            % Panoster & $84.0$ & $18.5$ & $36.4$ & $44.7$ & $30.1$ & $61.1$ & $69.2$ & $51.1$ & $90.2$ & $62.5$ & $34.5$ & $6.1$ & $82.0$ & $77.7$ & $55.7$ & $41.2$ & $48.0$ &  $48.9$ & $59.8$ & $52.7$ \\
            Panoptic-PolarNet & $88.8$ & $33.0$ & $51.8$ & $35.2$ & $37.6$ & $57.3$ & $69.9$ & $52.4$ & $88.6$ & $42.6$ & $\mathbf{61.2}$ & $1.6$ & $85.7$ & $46.0$ & $\mathbf{75.7}$ & $\mathbf{54.5}$ & $41.5$ & $48.5$ & $56.4$ & $54.1$ \\
            DS-Net & $91.2$ & $28.8$ & $45.4$ & $47.2$ & $34.6$ & $63.6$ & $71.1$ & $58.5$ & $89.1$ & $61.2$ & $32.3$ & $4.0$ & $83.2$ & $79.6$ & $58.3$ & $43.4$ & $50.0$ & $55.2$ & $\mathbf{65.3}$ & $55.9$ \\
            EfficientLPS & $85.7$ & $30.3$ & $37.2$ & $47.7$ & $43.2$ & $70.1$ & $66.0$ & $44.7$ & $\mathbf{91.1}$ & $\mathbf{71.1}$ & $55.3$ & $\mathbf{16.3}$ & $\mathbf{87.9}$ & $\mathbf{80.6}$ & $52.4$ & $47.1$ & $53.0$ & $48.8$ & $61.6$ & $57.4$ \\
            GP-S3Net & $84.1$ & $36.7$ & $41.8$ & $\mathbf{77.0}$ & $42.1$ & $73.0$ & $\mathbf{81.1}$ & $\mathbf{84.2}$ & $\mathbf{91.1}$ & $64.5$ & $38.9$ & $11.9$ & $80.4$ & $68.1$ & $53.2$ & $37.2$ & $46.9$ & $\mathbf{55.7}$ & $72.4$ & $60.0$ \\
            Panoptic-PHNet & $\mathbf{94.0}$ & $45.1$ & $\mathbf{54.6}$ & $62.4$ & $\mathbf{51.2}$ & $74.4$ & $76.3$ & $52.0$ & $89.9$ & $70.6$ & $49.4$ & $11.7$ & $87.8$ & $79.4$ & $57.2$ & $45.0$ & $52.6$ & $54.5$ & $61.2$ & $61.5$ \\
            
            \midrule
            \ours (ours) & $90.4$ & $\mathbf{45.9}$ & $47.3$ & $70.3$ & $45.1$ & $\mathbf{76.3}$ & $80.6$ & $69.8$ & $89.0$ & $68.7$ & $48.7$ & $6.0$ & $85.8$ & $79.5$ & $60.9$ & $46.1$ & $\mathbf{53.4}$ & $53.1$ & $64.9$ & $\mathbf{62.2}$\\
            \bottomrule
        \end{tabular}
    \end{center}
\end{table*}

==> tables/sem_val_classwise.tex <==
\begin{table*}[htbp]
\setlength\tabcolsep{2.5pt}
\begin{center}
\caption{Class-wise PQ, SQ, RQ on SemanticKITTI validation set. All scores are in [\%].}
        \label{tab:sem_test_classwise}
        \footnotesize
        \begin{tabular}{c|cccccccc|ccccccccccc|c}
            \toprule
            \begin{sideways}Metric\end{sideways} & \begin{sideways}car\end{sideways} & \begin{sideways}truck\end{sideways} & \begin{sideways}bicycle\end{sideways} & \begin{sideways}motorcycle\end{sideways} & \begin{sideways}other vehicle\end{sideways} & \begin{sideways}person\end{sideways} & \begin{sideways}bicyclist\end{sideways} & \begin{sideways}motorcyclist\end{sideways} & \begin{sideways}road\end{sideways} & \begin{sideways}sidewalk\end{sideways} & \begin{sideways}parking\end{sideways} & \begin{sideways}other ground\end{sideways} & \begin{sideways}building\end{sideways} & \begin{sideways}vegetation\end{sideways} & \begin{sideways}trunk\end{sideways} & \begin{sideways}terrain\end{sideways} & \begin{sideways}fence\end{sideways} & \begin{sideways}pole\end{sideways} & \begin{sideways}traffic sign\end{sideways} & \begin{sideways}Mean\end{sideways} \\
            \midrule
            \rowcolor[HTML]{D2FFFF}
            PQ & $93.1$ & $80.5$ & $68.9$ & $78.3$ & $68.2$ & $85.8$ & $92.1$ & $17.2$ & $93.7$ & $78.2$ & $27.3$ & $0.0$ & $88.8$ & $89.1$ & $56.9$ & $62.7$ & $25.4$ & $58.8$ & $58.5$ & $64.4$\\
            SQ & $94.8$ & $94.6$ & $82.3$ & $92.3$ & $93.9$ & $91.8$ & $93.5$ & $97.9$ & $93.7$ & $84.3$ & $73.5$ & $0.0$ & $91.1$ & $89.1$ & $74.8$ & $77.7$ & $73.1$ & $75.3$ & $75.5$ & $81.5$\\
            RQ & $98.2$ & $85.1$ & $83.7$ & $84.8$ & $72.6$ & $93.6$ & $98.5$ & $17.6$ & $100.0$ & $92.8$ & $37.1$ & $0.0$ & $97.5$ & $100.0$ & $76.1$ & $80.7$ & $34.8$ & $78.1$ & $77.4$ & $74.1$ \\
            \bottomrule
        \end{tabular}
    \end{center}
\end{table*}
